A General-Purpose Self-Supervised Model for Computational Pathology

Tissue phenotyping is a fundamental computational pathology (CPath) task in learning objective characterizations of histopathologic biomarkers in anatomic pathology. However, whole-slide imaging (WSI) poses a complex computer vision problem in which the large-scale image resolutions of WSIs and the enormous diversity of morphological phenotypes preclude large-scale data annotation. Current efforts have proposed using pretrained image encoders with either transfer learning from natural image datasets or self-supervised pretraining on publicly-available histopathology datasets, but have not been extensively developed and evaluated across diverse tissue types at scale. We introduce UNI, a general-purpose self-supervised model for pathology, pretrained using over 100 million tissue patches from over 100,000 diagnostic haematoxylin and eosin-stained WSIs across 20 major tissue types, and evaluated on 33 representative CPath clinical tasks in CPath of varying diagnostic difficulties. In addition to outperforming previous state-of-the-art models, we demonstrate new modeling capabilities in CPath such as resolution-agnostic tissue classification, slide classification using few-shot class prototypes, and disease subtyping generalization in classifying up to 108 cancer types in the OncoTree code classification system. UNI advances unsupervised representation learning at scale in CPath in terms of both pretraining data and downstream evaluation, enabling data-efficient AI models that can generalize and transfer to a gamut of diagnostically-challenging tasks and clinical workflows in anatomic pathology.

==> _dep/2.1-uni_overview_v1.tex <==

\heading{\ours: A Foundation Model for Representation Learning across Anatomic Pathology}
Here, we present \ours, a self-supervised, Vision Transformer (ViT) pretrained on over 100 million histopathology tissue patches across 100,000 H\&E WSIs and XXX tissue types. We demonstrate the versatility of \ours on a wide variety of machine learning regimes in computational pathology such as patch-level linear probing, full fine-tuning, few-shot learning, and as frozen feature extractors in slide-level weakly-supervised learning. In total, we assess \ours on 34 clinical tasks across anatomic pathology that range in clinical and technical difficulty, such as cell and tissue segmentation, primary and metastatic cancer detection, cancer grading and subtyping, gene mutation prediction and molecular subtyping, organ transplant assessment, and a curated 108-class OncoTree slide classification task. In developing \ours, we also investigate our model's scaling properties with respect to model size, dataset size and pretraining length, and show that scaling laws for self-supervised Vision Transformers in pathology emerge in solving challenging hierarchical classification tasks with increasing tissue diversity and disease categories. Below, we outline our methodology for developing and evaluating foundation models for CPATH, and our experimental setup on downstream tasks.

\hheading{OncoPath: A diverse dataset for histopathology image pretraining and Oncotree classification.} Observations and analyses of scaling laws in large language and vision models are owed to the development of large diverse datasets that have went beyond the imagination of current machine learning applications. For instance, ImageNet-22K (IN22K) is a hierarchical image database of 14.2 million images from 21,841 classes, with ImageNet-1K (IN1K) being a popular subset (1.2 million images, 1,000 classes) for self-supervised learning. Most similar to ImageNet as a dataset for image pretraining in CPATH is the TCGA, which contains XXX WSIs across XXX cancer types. However, many popular machine learning tasks constructed in CPATH are also derived from annotated histology slides in the TCGA, which limits the usability of current self-supervised models such as CTransPath and REMEDIS that utilize almost all histology slides in the TCGA for pretraining.

\noindent To train \ours, we curated our own in-house histology slide collection called "OncoPath", which we developed to be similar in tissue diversity to TCGA and in dataset size to current web-scale natural image datasets. Analogous to IN22K and IN1K, we developed a dataset called OP-22K, which contains 16 million histology image patches sampled from 21,444 WSIs across XXX tissue types and 354 unique OncoTree codes, as well as its subset OP-1K (1 million images, 1404 WSIs, XXX tissue types and XXX OncoTree codes). Analogous to even larger natural image datasets such as LVD-142M and JFT-300M used for observing scaling laws, we developed OP-100K, which combines OP-16M with further in-house slide collections and includes GTEx, a public biobank that contains 23XXX WSIs from 54 non-diseased tissue sites. We purposefully excluded using other public histology slide collections such as TCGA, CPTAC and PAIP for external evaluation of \ours. Altogether, OP-100M contains over 100 million histology images sampled from 100,000 WSIs and XXX tissue types.

% These datasets were developed to readily adapt successful self-supervised recipes for IN-1K and IN-22K into pathology data, as hyper-parameters may not immediately transfer well to larger datasets.

% Datasets such as CAMELYON16 and PANDA have enabled the development of recent FDA-approved pathology AI algorithms, but are limited to a single organ with few unique disease classes. Most similar to ImageNet in CPATH is TCGA,



% , though datasets such as CAMELYON16 and PANDA which have enabled the development of recent FDA-approved pathology AI algorithms, these datasets are limited to a single organ with limited disease classes. Moreover, the difficulty of these tasks may not be reflective 
\noindent To evaluate the generalizability of \ours on diverse tissue types, from the OP-1M subset, we constructed a hierarchical histology slide classification task similar in label scale to IN-1K called OP-108, a diverse 108-class OncoTree slide classification task of 2160 WSIs from 43 cancer types of both primary and metastatic origins, with each OncoTree code evenly represented with 20 labeled WSIs. We pose OP-108 as a few-shot learning problem, with 5 and 15 samples from each OncoTree code used in training and testing respectively. Additionally, we use the parent nodes in the OP-108 hierarchy to construct additional tasks for evaluation, such as OP-43 (43-way cancer type classification) and OP-2 (primary versus metastatic origin prediction). We refer readers to the \textbf{Online Methods} for more detailed reporting of the development and label distribution of OncoPath.

% We used OP-108 as a validation measure in our iterative pipeline for building a large-scale foundation model for pathology, similar to the way that IN-1K is routinely used for monitoring self-supervised performance. 


\hheading{Self-supervised pretraining for Vision Transformers.} For self-supervised learning, we experimented using DINOv2, which is a method based on student-teacher knowledge distillation for pretraining ViTs. In comparison to other self-supervised methods, an important property for pretrained vision models in histopathology is linear probe performance, as these models are often used as frozen feature extractors for pre-extracting patch features in a weakly-supervised slide-level tasks, with full-finetuning in patch-level tasks also not always feasible as collecting annotations can be costly and laborious. We used a ViT-Large with a $16 \times 16$ patch token size as our vision backbone due to it's demonstrated capabilities in scaling with increasing dataset size, as well as having emergent capabilities in understanding the semantic layout of histopathology images when pretrained using knowledge distillation. Altogether, \ours is a ViT-L/16 model pretrained using the DINOv2 recipe on our in-house OP100M dataset (excluding certain in-house subsets used for evaluation such as OP-108 and BWH-EMB). Experimentation and validation of scaling laws across smaller dataset sizes (OP1M and OP16M) and model sizes (ViT-S/16 and ViT-B/16) was conducted using the OP-2/43/108 slide classification tasks. We refer readers to the \textbf{Online Methods} for more detailed reporting regarding description of iBOT, DINOv2, and their pretraining hyper-parameters for different model and data sizes.

\hheading{Downstream evaluation, experimental setup, and baseline comparisons.} Following the development of \ours, we investigate it's capabilities across a range of 34 downstream tasks in CPATH in addition to OP-108 subtyping which include: CAMELYON16 (cancer detection), PANDA (Gleason score grading), TCGA Uniform Tumor (32-way pan-cancer classification), SegPath (8-class cell segmentation), and BWH-EMB (multi-task, in-house cardiac transplant assessment). To evaluate \ours on an external task that is similar to OP-2/43/108 subtyping in label complexity, we used the TCGA-GBMLGG cohort and the eBRAINS Digital Tumor Atlas to construct a 2-way \textit{IDH1} mutation prediction task, a 5-way histomolecular subtyping task, a 12-way cancer subtyping task, and a 24-way OncoTree subtyping task. We compare \ours to current publicly-available pretrained encoders used in routine experimentation in CPATH: 1) ResNet-50 with ImageNet Transfer, 2) CTransPath, 3) and REMEDIS. Patch-level classification tasks were evaluated using linear probing, nearest neighbors and few-shot evaluation, with patch-level segmentation tasks evaluated using full-finetuning and slide-level tasks evaluated using Attention-Based Multiple Instance Learning (ABMIL). We note that in some downstream tasks, as CTransPath and REMEDIS were trained using all of TCGA, the evaluation of these models should be viewed within a transductive setting. A detailed description of all tasks and their evaluation settings are described in the \textbf{Online Methods}.


% When possible, we used independent test cohorts for evaluating models trained on the TCGA, though many annotations for patch classification and segmentation tasks are completely derived using TCGA histology slides.
% We note that iBOT and DINOv2 are technically similar as they both use student-teacher distillation and masked image modeling losses, with DINOv2 extending the training recipe of iBOT further for larger models. For ablation experiments using models smaller than ViT-L/16, we use iBOT.
% To develop a foundation model for general representaiton learning across the 
% \noindent\textbf{2.1.3. OP-108 Subtyping: A 108-way/5-shot Oncotree slide classification task.} The observation and analysis of scaling laws in large language and vision models is owed to the development of large diverse datasets that have went beyond the imagination of modern machine learning applications. For instance, ImageNet-22K (IN22K) is a hierarchical image database of 14.2 million images from 21,841 classes, with ImageNet-1K (IN1K) being a popular subset (1.2 million images, 1,000 classes) for self-supervised learning. Datasets such as CAMELYON16 and PANDA have enabled the development of recent FDA-approved pathology AI algorithms, but are limited to a single organ with few unique disease classes. Most similar to ImageNet in CPATH is TCGA,

==> sections/0-abstract.tex <==
% \begin{spacing}{1.38}
% % The lack of annotated publicly available medical images is a major barrier for innovations. At the same time, many de-identified images and much knowledge are shared by clinicians on public forums such as medical Twitter. Here we harness these crowd platforms to curate OpenPath, a large dataset of 208,414 pathology images paired with natural language descriptions. This is the largest public dataset for pathology images annotated with natural text. We demonstrate the value of this resource by developing PLIP, a multimodal AI with both image and text understanding, which is trained on OpenPath. PLIP achieves state-of-the-art zero-shot and transfer learning performances for classifying new pathology images across diverse tasks. Moreover, PLIP enables users to retrieve similar cases by either image or natural language search, greatly facilitating knowledge sharing. Our approach demonstrates that publicly shared medical information is a tremendous resource that can be harnessed to advance biomedical AI.
% % Mapping gene networks requires large amounts of transcriptomic data to learn the connections between genes, which impedes discoveries in settings with limited data, including rare diseases and diseases affecting clinically inaccessible tissues. Recently, transfer learning has revolutionized fields such as natural language understanding1,2 and computer vision3 by leveraging deep learning models pretrained on large-scale general datasets that can then be fine-tuned towards a vast array of downstream tasks with limited task-specific data. Here, we developed a context-aware, attention-based deep learning model, Geneformer, pretrained on a large-scale corpus of about 30 million single-cell transcriptomes to enable context-specific predictions in settings with limited data in network biology. During pretraining, Geneformer gained a fundamental understanding of network dynamics, encoding network hierarchy in the attention weights of the model in a completely self-supervised manner. Fine-tuning towards a diverse panel of downstream tasks relevant to chromatin and network dynamics using limited task-specific data demonstrated that Geneformer consistently boosted predictive accuracy. Applied to disease modelling with limited patient data, Geneformer identified candidate therapeutic targets for cardiomyopathy. Overall, Geneformer represents a pretrained deep learning model from which fine-tuning towards a broad range of downstream applications can be pursued to accelerate discovery of key network regulators and candidate therapeutic targets.
% Tissue phenotyping is a fundamental computational pathology (CPath) task in learning objective characterizations of histopathologic biomarkers in anatomic pathology. However, whole-slide imaging (WSI) poses a complex computer vision problem in which the large-scale image resolutions of WSIs and the enormous diversity of morphological phenotypes preclude large-scale data annotation.  To address these limitations, current efforts have proposed using pretrained image encoders with either transfer learning from a natural image dataset or self-supervised pretraining on a publicly-available histopathology dataset, in extracting morphological features from WSIs, but have not been extensively developed and evaluated across diverse tissue types. In this work, we introduce a new foundation model, or a general-purpose vision backbone, for pathology, called \ours, based on self-supervised Vision Transformers. \ours is pretrained using over 100 million tissue patches sampled across X tissue types and 100,000 diagnostic haematoxylin and eosin-stained WSIs, and evaluated with over 33 representative benchmarks in Cpath, such as lymph node metastasis detection, Gleason score grading, and other clinical tasks such as mutation prediction, cell detection and segmentation that span multiple tissue types. By pretraining on large-scale and diverse tissue patches, \ours outperforms other state-of-the-art pretrained CPath models across many different tasks and transfer learning scenarios such as region-of-interest classification, retrieval, and segmentation, as well as WSI classification, while being data-efficient. 
% % multiple instance learning, linear probing, end-to-end finetuning, and few-shot learning. 
% Overall, we demonstrate the capabilities of \ours as a foundation model for developing AI models in anatomic pathology.
% \end{spacing}

==> sections/__dep__2.1-uni_overview.tex <==

\heading{\ours: A Foundation Model for Representation Learning across Anatomic Pathology}

\noindent
% We demonstrate the versatility of \ours in various machine learning regimes in CPath, such as patch-level linear probing, full fine-tuning, few-shot learning, and as a frozen feature extractor in slide-level weakly-supervised learning (\textbf{Figure \ref{fig:overall}A}). 
%We demonstrate the versatility of \ours in diverse machine learning settings within CPath, including region-of-interest (ROI)-level classification, segmentation and image retrieval, and slide-level weakly-supervised and semi-supervised learning (\textbf{Figure \ref{fig:overall}C}). Specifically, we assess \ours on 33 clinical tasks across anatomic pathology that range in clinical and technical difficulty, such as nuclear segmentation, primary and metastatic cancer detection, cancer grading and subtyping, gene mutation prediction and molecular subtyping, organ transplant assessment, and a curated 108-class OncoTree slide classification task (\textbf{Figure \ref{fig:overall}d}).
% In developing \ours, we also investigate our model's scaling properties with respect to dataset size and pretraining length and show that scaling laws for self-supervised Vision Transformers in pathology emerge in solving challenging hierarchical classification tasks with increasing tissue diversity and disease categories.
% We also investigate our model's scaling properties when increasing the dataset size, tissue diversity, and pretraining time. Our results show that the performance of self-supervised Vision Transformers in pathology follows scaling laws, which become particularly apparent when evaluating on complex hierarchical classification tasks. Below, we outline our methodology for developing and evaluating foundation models for CPath across a diverse range of tasks.

\hheading{OncoPath: A diverse dataset for histopathology image pretraining and Oncotree classification.}

The transfer learning and generalization capabilities of self-supervised models are intrinsically tied to the size and diversity of the training data. In computer vision, foundation models were originally developed using ImageNet\cite{deng2009imagenet}, starting with ImageNet-1K (IN-1K) encompassing 1.2 million images from 1,000 classes, followed by ImageNet-22K (IN-22K, 14.2 million images from 21,841 classes), and then even larger datasets such as LVD-142M and JFT-300M. In CPath, The Cancer Genome Atlas (TCGA, $\sim$11,000 FFPE H\&E WSIs, 32 cancer types) serves as the basis for most self-supervised models~\cite{wang2021transpath,chen2022scaling,wang2022transformer,azizi2023robust, kang2023benchmarking}, but has from several limitations as a pretraining data source. As many popular clinical tasks in CPath are also based on annotated histology slides from TCGA, current self-supervised models pretrained on TCGA are not suitable for routine CPath benchmarks and lack extensive evaluation of out-of-domain generalization performance~\cite{wang2021transpath,wang2022transformer}. In terms of tissue diversity, the TCGA is mostly comprised of slides with invasive malignancies from common primary sites, and thus may not encompass sufficient phenotypic variability found in broad anatomical pathology practice.

% Observations and analyses of scaling laws in foundation models are owed to developing large, diverse datasets that have gone beyond the imagination of current machine learning applications. For instance, ImageNet-22K (IN-22K) is a hierarchical image database of 14.2 million images from 21,841 classes, with ImageNet-1K (IN-1K) being a popular subset (1.2 million images, 1,000 classes) for self-supervised learning. Most similar to ImageNet as a dataset for image pretraining in CPATH is The Cancer Genome Atlas (TCGA), which contains XXX WSIs across XXX cancer types. However, many popular CPATH machine learning tasks constructed are also derived from annotated histology slides in the TCGA, which limits the usability of current self-supervised models that utilize TCGA histology slides for pretraining (cite  CTransPath and REMEDIS).

\noindent To develop a foundation model that can generalize across routine clinical tasks in CPath, we curated a large histology slide collection termed \textit{OncoPath}, comprised of in-house histology slides from Massachusetts General Hospital and Brigham \& Women's Hospital, and external histology slides from the Genotype-Tissue Expression (GTEx) consortium. Following natural image datasets, we also created three partitions of OncoPath that vary in size in order to evaluate the data scaling laws, an empirical observation found in natural language and image foundation models that scaling dataset size would also increase model performance. Analogous to IN-22K and IN-1K, we developed the OP-22K dataset, which contains 16 million histology image patches sampled from 21,444 WSIs across 20 major tissue types with cancerous tissue, as well as its subset OP-1K (1 million images, 1,404 WSIs). Inspired by the massive dataset sizes of LVD-142M and JFT-300M, we developed OP-100K, which contains over 100 million histology images sampled from 100,000 WSIs, which combines OP-22K with further in-house slide collections and GTEx which is comprised of non-cancerous 24,782 WSIs. We purposefully excluded using other public histology slide collections such as TCGA, CPTAC, and PAIP for external evaluation of \ours. Altogether, we use OP-1K, OP-22K, and OP-100K in our development of general-purpose self-supervised models


% and the dataset size of current web-scale natural image datasets, for training \ours.

% \TODO{Immediate todo for Richard: Add table for OP-1K and OP-22K. Getting final counts. Follow Drew's suggestions in Slack channel on: "we can be a bit more wishy-washy int eh text and just say something like "we train on tissue cover every tissue site at the top level of OncoTree--32 sites--including both cancerous and non-cancerous lesional tissue as well as normal tissue from all sites}


\hheading{Self-supervised pretraining for Vision Transformers.} $\ours$ is a ViT-Large architecture pretrained on OncoPath using DINOv2~\cite{oquab2023dinov2}, which is a state-of-the-art self-supervised learning paradigm based on student-teacher knowledge distillation~\cite{grill2020bootstrap, caron2021emerging} and masked image modeling~\cite{zhou2021ibot} (\textbf{Fig. \ref{fig:overall}b}). DINOv2 employs a contrastive and reconstruction loss function to encourage the student network to match the representations of patches to those generated by a slowly updating teacher model. Compared to other types of self-supervised methods~\cite{he2022masked,tian2022designing}, pre-extracted representations from DINOv2 exhibit high classification performance without the need for further fine-tuning. This property holds particular significance in CPath, as most slide classification approaches rely on transfer learning by extracting patch embeddings from pretrained, frozen feature extractors. 


% We refer readers to the \textbf{Online Methods} for more detailed reporting regarding description of iBOT, DINOv2, and their pretraining hyper-parameters for different model and data sizes.



% Compared to other self-supervised methods, an important property for pretrained vision models in histopathology is linear probe performance, as these models are often used as frozen feature extractors for pre-extracting patch features in weakly-supervised slide-level tasks, with full-finetuning in patch-level tasks also not always feasible as collecting annotations can be costly and laborious.
%  @TODO: do we want that here?
% Specifically, when training on OP-100K, we used a ViT-Large architecture with a $16 \times 16$ patch token size as our primary vision backbone due to its demonstrated capabilities in scaling with increasing dataset size, as well as having capabilities in understanding the semantic layout of histopathology images when pretrained using knowledge distillation.

% cut bits and pieces:
% Here, we present \ours, a self-supervised Vision Transformer (ViT) pretrained on over 100 million histopathology tissue patches across 100,000 H\&E WSIs and XXX tissue types. 

% Experimentation and validation of scaling laws across smaller dataset sizes (OP1M and OP16M) and model sizes (ViT-S/16 and ViT-B/16)



% We refer readers to the \textbf{Online Methods} for more detailed reporting regarding description of iBOT, DINOv2, and their pretraining hyper-parameters for different model and data sizes.



% When possible, we used independent test cohorts for evaluating models trained on the TCGA, though many annotations for patch classification and segmentation tasks are completely derived using TCGA histology slides.
% We note that iBOT and DINOv2 are technically similar as they both use student-teacher distillation and masked image modeling losses, with DINOv2 extending the training recipe of iBOT further for larger models. For ablation experiments using models smaller than ViT-L/16, we use iBOT.
% To develop a foundation model for general representaiton learning across the 
% \noindent\textbf{2.1.3. OP-108 Subtyping: A 108-way/5-shot Oncotree slide classification task.} The observation and analysis of scaling laws in large language and vision models is owed to the development of large diverse datasets that have went beyond the imagination of modern machine learning applications. For instance, ImageNet-22K (IN22K) is a hierarchical image database of 14.2 million images from 21,841 classes, with ImageNet-1K (IN1K) being a popular subset (1.2 million images, 1,000 classes) for self-supervised learning. Datasets such as CAMELYON16 and PANDA have enabled the development of recent FDA-approved pathology AI algorithms, but are limited to a single organ with few unique disease classes. Most similar to ImageNet in CPATH is TCGA,
